Foundations of Platform-Assisted Auctions

Today, many auctions are carried out with the help of intermediary platforms like Google and eBay. We refer to such auctions as platform-assisted auctions.Traditionally, the auction theory literature mainly focuses on designing auctions that incentivize the buyers to bid truthfully,assuming that the platform always faithfully implements the auction. In practice, however, the platforms have been found to manipulate the auctions to earn more profit, resulting in high-profile anti-trust lawsuits. We propose a new model for studying platform-assisted auctions in the permissionless setting. We explore whether it is possible to design a dream auction in thisnew model, such that honest behavior is the utility-maximizing strategy for each individual buyer, the platform, the seller, as well as platform-seller or platform-buyer coalitions.Through a collection of feasibility and infeasibility results,we carefully characterize the mathematical landscape of platform-assisted auctions. We show how cryptography can lend to the design of an efficient platform-assisted auction with dream properties. Although a line of works have also used MPC or the blockchain to remove the reliance on a trusted auctioneer, our work is distinct in nature in several dimensions.First, we initiate a systematic exploration of the game theoretic implications when the service providers are strategic and can collude with sellers or buyers. Second, we observe that the full simulation paradigm is too stringent and leads to high asymptotical costs. Specifically, because every player has a different private outcomein an auction protocol, running any generic MPC protocol among the players would incur at least $n^2$ total cost. We propose a new notion of simulation calledutility-dominated emulation.Under this new notion, we showhow to design efficient auction protocols with quasilinear efficiency.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

TARGET=platform-auction.pdf 
#TARGET2=leader-election-llncs.pdf 

#all: $(TARGET) $(TARGET2)
all: $(TARGET)
 

$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
#	bibtex $(basename $<)
#	bibtex $(basename $<)
#	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<


full: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<


$(TARGET2): $(TARGET2:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex leader-election-llncs
	bibtex leader-election-llncs
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<



test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.out *.log *.aux *.bbl *.blg *.bak .*.xtx.cache parsetab.py \#*\# *~


==> crypto-constr-elaine.tex <==


\section{Compiling an Ideal Auction to a Cryptographic Protocol}
\label{sec:real-world}
\elaine{TO FIX: subtle issue, if platform does not send n, we need
AoK for TM, need to add it}

\subsection{Compiler}

\elaine{TODO: added coin toss into protocol, not proof yet}

\paragraph{Building blocks.} 
We will rely on 
a family $\mcal{F}_{\rm hash}$ of coalition resistant hash functions 
that map arbitrary-length strings to a $\lambda$-bit digest, 
a non-interactive, computationally hiding and 
perfectly binding commitment scheme $\Comm$, %\hao{Do we need perfectly binding?} 
a non-interactive zero-knowledge proof system $\NIZK$,
and an interactive succinct argument of knowledge scheme $\AoK$.
We will need to use the $\AoK$ to prove
four different languages, so we denote the four instances
of $\AoK$ as $\AoK_1$, $\AoK_2$, $\AoK_3$ and $\AoK_4$ respectively.  

\paragraph{NP languages.} 
We now specify the NP languages $\mcal{L}_0^\lambda,
 \mcal{L}_1^\lambda,\mcal{L}_2^\lambda,\mcal{L}_3^\lambda, \mcal{L}_4^\lambda$ 
we will need  
for running $\NIZK$ and the four $\AoK$ instances $\AoK_1$, $\AoK_2$, $\AoK_3$ and $\AoK_4$, respectively. 
Henceforth, we shall assume that a common reference
string $\crs$
and a randomly selected hash function $h$
is clear from the context, so we need not explicitly include
it in the statements.  

\elaine{TODO: FIX: Comm needs to take lambda}

\begin{enumerate}[leftmargin=8mm,itemsep=1pt]
\item[0.]
%\elaine{TO FIX: i can commit to not my id}
A statement $(i, c)$ is in $\mcal{L}_0^\lambda$ 
if $\exists$ a witness $(\msg, \coin)$ such that 
$\Comm(1^\lambda, i\|\msg; \coin) = c$.
%\hfill{\it//~buyer proves to platform}
\item 
A statement $(\digest, i, c_i,\pi_i)$ is in $\mcal{L}_1^\lambda$ 
if $\exists$ a witness $(\bfc, r_{\platform})$ such that
%\ \  \hfill{\it//~platform proves to buyer}
\begin{enumerate}[itemsep=1pt]
    \item $(i, c_i, \pi_i) \in \bfc$; \elaine{TODO: fix all the order}
    \item $\digest = h(\bfc\|r_{\platform})$; 
    \item All tuples in $\bfc$ contain distinct identities.
    \item $\NIZK.\Ver(\NIZKcrs, (j, c_j), \pi_j) = \acc$ 
for all $(j, c_j, \pi_j) \in \bfc$.
\hfill {\it // The NIZK language is $\mcal{L}_0^\lambda$}.
\end{enumerate}
\item 
A statement $\digest$ is in $\mcal{L}_2^\lambda$ if there exists 
a witness  $(\bfc, r_\platform)$ such that
(b)-(d) of $\mcal{L}_1^\lambda$ hold. 

\elaine{hard-coded refs}  
%\begin{itemize}
%    \item $\digest = h(\bfc)$;
%    \item All tuples in $\bfc$ contain distinct identities.
%    \item $\NIZK.\Ver(\NIZKcrs, c_j, \pi_j) = \acc$ for all $(c_j, j, \pi_j) \in \bfc$.
%\elaine{TODO: fix here}
%\end{itemize}
\item 
A statement $(\digest, x_i, p_i)$ is in $\mcal{L}_3^\lambda$ 
if $\exists$ 
a witness $(\mcal{I}, 
\bfc= \{(j, c_j, \pi_j)\}_{j\in \mcal{I}}, 
\{(v_j, r_j,  \coin_j)\}_{j\in \mcal{I}}, r_\platform
)$ 
such that
\elaine{TODO: change witness format to be consistent}
\begin{enumerate}[itemsep=1pt]
    \item $\digest = h(\bfc\|r_\platform)$;
    \item $\Comm(1^\lambda,j\|v_j\|r_j; \coin_j) = c_j$ for all %$(c_j, j, \pi_j) \in \bfc$;
$j \in \mcal{I}$;  
    \item $x_i = \bfx_i(1^\lambda, \bfv; r)$ 
and $p_i = \bfp_i(1^\lambda, \bfv; r)$ 
where $r = 
\left(\displaystyle\mathop{\oplus}_{j \in \mcal{I}} r_j\right) \oplus r_\platform$
 and $\bfv = \{v_j\}_{j\in \mcal{I}}$.
%	That is, $(x_i, p_i)$ is computed based on the rule $(\bfx,\bfp)$ using the bids $\bfv$ and the randomness $\bfr_{\platform}$.
\end{enumerate}
Here, $\bfx_i(1^\lambda, \bfv; \bfr_{\platform})$
means that we run the allocation  
rule ${\bf x}$ with input $\bfv$ and randomness
$r$ and output the coordinate that encodes
the bid of the identity $i$; and 
$\bfp_i(1^\lambda, \bfv; \bfr_{\platform})$
is similarly defined. 
\item 
A statement $(\digest, \mu, t)$ 
is in $\mcal{L}_4^\lambda$ if $\exists$ 
a witness $(\mcal{I}, 
\bfc= \{(j, c_j, \pi_j)\}_{j\in \mcal{I}}, 
\{(v_j, r_j,  \coin_j)\}_{j\in \mcal{I}}, r_\platform
)$ 
such that
\begin{itemize}[itemsep=1pt]
\item 
(a) and (b) of $\mcal{L}_3^\lambda$ hold, and 
\item $t = \sum_{j \in \mcal{I}}\bfx_{j}(1^\lambda, \bfv;r)$ 
and $\mu = \mu_{\mcal{S}}(1^\lambda, \bfv;r)$
    where 
$\left(\displaystyle\mathop{\oplus}_{j \in \mcal{I}} r_j\right) \oplus r_\platform$, and
$\bfv = \{v_j\}_{j\in \mcal{I}}$.
That is, $(t, \mu)$ is computed based on the rule 
$(\bfx,\mu_{\mcal{S}})$ using the bids $\bfv$ and 
the randomness $r$ as input.
\end{itemize}
\end{enumerate}
% \hao{TODO: clarify the auction rules and private outcome.}


\paragraph{Compiler.} 
We assume every buyer is associated with a distinct identity.
However, the strategic players, including the platform, the seller, or buyers,
may additionally choose fake identities and pretend to be multiple buyers. 
%\hao{Sample identities.}

Given an ideal-world auction $\Pi^\Ideal_\lambda[{\bf x}, {\bf p}, \mu_{\mcal{S}}]$, 
\elaine{I added sec param, make all consistent}
we can compile it to a real-world auction 
$\Pi^\Real_\lambda[{\bf x}, {\bf p}, \mu_{\mcal{S}}]$
as follows. 


\begin{mdframed}
\begin{center}
{\bf Real-world auction $\Pi^\Real_\lambda[{\bf x}, {\bf p}, \mu_{\mcal{S}}]$} 
\end{center}
\vspace{5pt}
% \noindent {\bf Parameters:} The security parameter $\secu$, and a common reference string ${\sf crs}=(\crs_c,\crs_p)$ where $\crs_c$ and $\crs_p$ are generated by the common-reference-string generation algorithm of ${\sf Comm}$ and ${\sf SNARG}$, respectively.

\noindent {\bf Inputs:} 
Each buyer has a true value from $\inDomSecu$. All players hold the security parameter $1^\secu$.

\vspace{5pt} \noindent {\bf Setup:}
\begin{enumerate}[leftmargin=6mm]
\item[] 
Sample a random hash function $h \leftarrow \mcal{F}_{\rm hash}^\lambda$, 
\elaine{parametrized by lambda now, change prelim}
common reference strings
$\NIZKcrs \leftarrow \NIZK.\Gen(1^\secu, \mcal{L}_0)$.
% for $j \in [4]$, sample 
% $\crs_j \leftarrow \AoK_j.\Gen(1^{\secu}, \mcal{L}_j)$. 
Publish the public parameters 
including $\NIZKcrs$ and a description of $h$.
\end{enumerate}

\vspace{5pt} \noindent {\bf Main auction protocol:}
\elaine{TODO: fix: many crypto primitives don't take lambda,
Pi also should take lambda}
\begin{enumerate}[leftmargin=6mm]
\item 
%Each buyer $i$ randomly samples its identity $\id_i \leftarrow \{0,1\}^{\secu}$, 
% Each buyer samples a random identity $i \leftarrow \{0, 1\}^\secu$, 
% prepares a bid $b_i$ according to the bidding rule of $\Pi$,
Each buyer $i$ samples
$r_i\getr \{0,1\}^\lambda$, 
computes the commitment $c_i \leftarrow \Comm(1^\lambda, i\|v_i\|r_j; \coin_i)$
where $\coin_i$ are freshly sampled random coins of appropriate length.
Then, buyer $i$ generates a proof 
$\pi_i \leftarrow \NIZK.\Prove(\NIZKcrs, (i, c_i), (v_i\|r_i, \coin_i))$ 
for the statement $(i, c_i)$ using the witness $(v_i\|r_i, \coin_i)$. 
Finally, buyer $i$ sends $(i, c_i, \pi_i)$ to the platform.
\item
\label{stp:hash}
The platform ignores all the tuples $(i, c_i, \pi_i)$ where $\NIZK.\Ver(\NIZKcrs, (i, c_i), \pi_i) = \rej$.
Among the remaining tuples, 
if there are multiple tuples containing the same identity $i$,
the platform randomly keeps one of the tuples and ignores the rest.
For each identity ignored, the platform notifies
the corresponding buyer,  
and the corresponding buyer rejects the auction. 

\hao{random selection for symmetry.}

Let $\bfc = \{(i, c_i, \pi_i)\}_{i \in \mcal{I}}$
be the remaining tuples where $\mcal{I}$ denotes 
the identities they are associated with. 
The platform samples randomness $r_{\platform}$,
sends $\digest = h(\bfc\|r_\platform)$ to all buyers and the seller.
\item
\label{stp:proof-commitment}
% For each buyer $i$, the platform generates a proof for statement $(h, c_i, \id_i)$ 
% using the witness $\bfc$, and $\bfr_{\platform}$ to prove that 
The platform and each buyer identity $i \in \mcal{I}$ invoke
$\AoK_1$ where the platform acts as the prover and proves
the statement $(\digest, i, c_i, \pi_i)$ is in $\mcal{L}_1$
using the witness $(\bfc, r_\platform)$. 
Similarly, the platform and the seller invoke $\AoK_2$ 
where the platform proves the statement $\digest$ is in $\mcal{L}_2$
using the witness $(\bfc, r_\platform)$. 
If the proof fails for any verifier, the verifier 
rejects the auction;
\item 
Every buyer $i$ %that did not reject 
sends the opening $(v_i\|r_i, \coin_i)$ to the platform.

\item
\label{stp:outcome}
Let $(v_i\|r_i, \coin_i)$ denote the 
opening received by the platform from buyer identity $i$. 
If for some $i \in \mcal{I}$, 
$(i\|v_i\|r_i, \coin_i)$ 
is not a correct opening of $c_i$ or $i$ did not respond,  
the platform posts $\bot$ to the blockchain, and all players reject. 
%\item 
Otherwise, 
the platform runs the 
auction's rules $({\bf x}, {\bf p}, \mu_{\mcal{S}})$
using the bid vector  $\{v_i\}_{i \in \mcal{I}}$ 
and the randomness $r = \left(\displaystyle\mathop{\oplus}_{i \in \mcal{I}} r_i\right) 
\oplus r_\platform $ as input,
and sends the private outcome $(x_i,p_i)$ to each buyer identity $i \in \mcal{I}$
and sends $(t,\mu_{\seller})$ to the seller.
\elaine{TO FIX: should platform also contribute randomness? does
our proof current work when all buyers are corrupt}
\item 
\label{stp:proof-auction}
The platform and each buyer $i \in \mcal{I}$ invoke
$\AoK_3$ where the platform proves
the statement 
% For each buyer $i$, the platform generates the proof for statement $(h, x_i,p_i)$ 
% using $\AoKcrs$ and the witness $\bfc$, $\bfr_{\platform}$, and $\{b_j\}_{\id_j\in \mcal{I}}$ to prove that
%For each buyer $i$, the platform as the prover and buyer $i$ as the verifier jointly invokes $\AoK$ for statement 
$(\digest, x_i,p_i)$ is in $\mcal{L}_3$
using the witness $(\mcal{I}, 
\bfc= \{(j, c_j, \pi_j)\}_{j\in \mcal{I}}, 
\{(v_j, r_j, \coin_j)\}_{j\in \mcal{I}}, r_\platform)$.  
% \elaine{move relation outside}
If the proof fails, buyer $i$ rejects the auction and aborts.

Similarly, the platform and the seller invoke $\AoK_4$ 
where the platform proves the statement $(\digest, t, \mu_S)$ is in $\mcal{L}_4$
using the witness 
$(\mcal{I}, \bfc= \{(j, c_j, \pi_j)\}_{j\in \mcal{I}}, 
\{(v_j, r_j, \coin_j)\}_{j\in \mcal{I}}, r_\platform)$.
If the proof fails, the seller rejects the auction and aborts. 
\item 
The platform posts the public outcome 
$h(\bfc\|r_\platform)$ to the blockchain.
Each buyer or seller checks whether the public outcome is 
the same as the hash value received in Step \ref{stp:hash}.
If so, output the private outcome received in Step \ref{stp:outcome};
otherwise, reject the auction.
\end{enumerate}
\end{mdframed}

% Let $\util^{\Ideal}_{\mcal{C}}(\trace)$ and $\util^{\Real}_{\mcal{C}}(\trace)$ denote the utility of $\mcal{C}$ given the execution trace
% $\trace$ in the ideal execution and real execution, respectively.
% Recall that when we fix any coalition $\coalition$, $\Ver(\trace) = \acc$ denotes the event that the trace is safe,
% i.e.~all honest players outside $\coalition$ accepts the auction in the trace $\trace$.
% Fix any bid vector $\bfb_{-\mcal{C}}$ submitted by the buyers outside $\coalition$.
% Let $\trace \leftarrow {\sf Exec}_{\Real}^S(\bfb_{-\mcal{C}})$ and $\trace \leftarrow {\sf Exec}_{\Ideal}^S(\bfb_{-\mcal{C}})$ denote
% the act of sampling a random execution trace in the real execution and the ideal execution, respectively,
% given that $\mcal{C}$ adopts the strategy $S$
% and every player outside $\mcal{C}$ plays honestly
% conditioned on using the input vector $\bfb_{-\mcal{C}}$.



\paragraph{Asymptotically efficient instantiation.}
We can instantiate the protocol using
a constant-round
 AoK protocol based on Probablistic Checkable Proofs (PCPs) 
such as Kilian~\cite{}. 
\elaine{add cites}
Further, we can use a PCP construction that has 
quasilinear-prover time~\cite{}. 
\elaine{add cites}
The resulting protocol has $O(1)$ number of rounds,
the platform's running time is $\widetilde{O}(n)$,
\elaine{TO FIX: THIS requires 1-to-many proofs,
it might only work for SNARK, or using extra coin toss
to have a shared random challenge, but not clear how to do this.
or use same PCP for everyone, and everyone challenges
different locations: defer to second step? 
just do it in the robust version}
and the seller and each buyer's running time  
is $\widetilde{O}(1)$, where $\widetilde{O}(\cdot)$ hides
polylogarithmic factors and factors 
dependent on the security parameter $\lambda$.   
%The above protocol can be based on 
Further, all of the building blocks rely on 
standard cryptographic assumptions.
\elaine{technicality: need commitment for expected poly time} 


\begin{remark}[More practical instantiation using SNARKs]
In practice, we can instantiate
the AoK instances using a state-of-the-art Succinct
Non-interactive
ARgument of Knowledge (SNARK)~\cite{}.
\elaine{TODO: add cites}
Observe that in this case, the 
seller does not need to actively send messages
in the protocol.
The resulting protocol has only four rounds. 

We chose to first present the protocol more generally using interactive AoK
since theoretically, it is interesting to get the result
from standard cryptographic assumptions.
In general, SNARKs
cannot be based on standard cryptographic assumptions~\cite{}.
\elaine{cite, make the statement more precise}
\end{remark}






\begin{theorem}[Real is a utility-dominated emulation of ideal]
\label{thm:IC-ideal-real}
Given an arbitrary ideal auction 
$\Pi_\lambda^\Ideal[{\bf x}, {\bf p}, \mu_{\mcal{S}}]$, 
%and suppose that at least 
%one buyer is not strategic or the platform is not strategic, then  
for any strategic $\mcal{C}$
that is either the seller, the platform, an individual 
buyer, the platform-seller
coalition, or a platform-buyer coalition, 
the real-world protocol
$\Pi_\lambda^\Real[{\bf x}, {\bf p}, \mu_{\mcal{S}}]$ is a utility-dominated
emulation of  
$\Pi_\lambda^\Ideal[{\bf x}, {\bf p}, \mu_{\mcal{S}}]$
w.r.t. $\mcal{C}$, as long as 
there is one non-strategic buyer 
or the platform is non-strategic. 

Further, if the ideal auction is deterministic, 
then the condition 
that at least one buyer or the platform is non-strategic can be removed.
\elaine{because of coin toss}
\label{thm:realemulates}
\end{theorem}
The formal proof of \cref{thm:realemulates} is provided 
in \cref{sec:thm:IC-ideal-real}.





==> cryptoproofs-elaine.tex <==

\subsection{Proof of \cref{thm:IC-ideal-real}}
\label{sec:thm:IC-ideal-real}

\elaine{NOTATION in the proof also needs to change to new version, fix proof for coin toss} 

%\subsubsection{Utility Equivalence under Honest Execution}
Suppose that the AoK and NIZK satisfy perfect completeness.
Then, it is easy to see that under honest execution, 
every player's utility in the ideal world 
is identically distributed as its utility 
in the real world. 
% has negligible statistical difference
% between the ideal- and real-world
% execution. 
% This is because conditioned on no identities colliding,
% the real-world utility is identically distributed as the ideal world. 
% Since honest players sample their identities at random from $\{0, 1\}^\lambda$,
% the probability of having a collision is negligibly small.
Next, we will focus on proving that 
for any real-world \ppt coalition strategy, there is a corresponding
ideal-world strategy such that 
the coalition's utility in the real world
%is $(1-\negl(\lambda))$-almost perfectly dominated
is  computationally dominated 
by its ideal-world utility. 


\subsubsection{Case 1: Platform is Strategic}
\label{sec:proof-strategic-platform}
We first prove for the case when the platform is part of the 
strategic coalition $\mcal{C}$.
Specifically, $\mcal{C}$ can be the platform alone,
the platform-seller
coalition, or a platform-buyer coalition with one or more buyers. 


\paragraph{Experiment $\Hyb_1$.}
$\Hyb_1$ is almost the same as the real-world protocol, 
except with the following modification. 
Instead of generating the $\NIZKcrs$ of $\NIZK$ honestly, 
we will call the simulated 
setup algorithm $(\NIZKcrs, \tau, \ek) \leftarrow \NIZK.\widetilde{\sf Gen}(1^\lambda, \mcal{L}_0)$
to generate a simulated $\NIZKcrs$ 
along with a trapdoor $\tau$ and an extraction key $\ek$. 
When honest buyers send to $\mcal{C}$ commitments 
of their true values along with a NIZK
proof,  we replace the honestly constructed NIZK proofs
with simulated proofs generated with the trapdoor $\tau$ without using the witness.  

\elaine{one or more of the claims implicitly use perfectly binding}

\begin{claim}
\label{claim:real-hyb1}
Suppose that $\NIZK$ satisfies 
computational zero-knowledge, 
and $\mcal{C}$ is probablistic polynomial-time, 
then $\mcal{C}$'s utility in the real-world execution 
is computationally indistinguishable
from $\Hyb_1$.  
\end{claim}
\begin{proof}
The proof follows from a straightforward reduction.  
\end{proof}


\paragraph{Experiment $\Hyb_2$.}
$\Hyb_2$ is almost the same as $\Hyb_1$
except that when $\mcal{C}$ executes  
an instance of $\AoK_1$ (for buyers) or $\AoK_2$ (for sellers)
%to prove knowledge of the opening of 
%${\sf digest}$ 
with the first honest player denoted $i^*$ (either a buyer or seller), 
\elaine{can also work for platform seller coalition}
we additionally invoke the corresponding knowledge extractor on the side 
to extract a witness 
${\bf c}||r_{\mcal{P}}$. 
Note that from the extractor's persective, 
the adversarial prover's circuit consists of  
the coalition $\mcal{C}$'s algorithm, random coins, its state 
at the beginning of the $\AoK_1$ or $\AoK_2$ instance,
as well as the verifier circuits and random coins of all other honest players 
except $i^*$ for the $\AoK_1$ or $\AoK_2$ instances.

Now, if player $i^*$ 
accepts the platform's proof %but $h({\bf c}||{\bf r}_{\mcal{P}})$ 
but 
${\bf c} \| r_\mcal{P}$
is not a valid witness to the statement,  
then the experiment aborts and 
the coalition $\mcal{C}$'s utility is treated as $0$. 
Otherwise, we 
parse 
${\bf c} := \{i, c_i, \pi_i\}_{i \in \mcal{I}}$, and 
invoke the $\NIZK$'s extractor 
which uses the extraction key $\ek$, and 
for each strategic buyer $j \in \mcal{I} \backslash \mcal{H}$ where $\mcal{H}$ denotes
the honest buyers, extract from $\pi_{j}$ 
the opening 
$(j \| v_j \| r_j, {\sf coin}_j)$. 
If there exists $j \in \mcal{I} \backslash \mcal{H}$ such that 
the extracted 
$(j \| v_j \| r_j, {\sf coin}_j)$ is not a valid opening of 
the commitment $c_j$, then abort and treat $\mcal{C}$'s utility as 0.

In $\Hyb_2$, the extracted 
${\bf c} := \{i, c_i, \pi_i\}_{i \in \mcal{I}}$, 
$r_{\mcal{P}}$, and  $\{(j \| v_j \| r_j, 
{\sf coin}_j)\}_{j \in \mcal{I} \backslash \mcal{H}}$ are not 
used so we just save the values on the side. 
These values will be referenced in later hybrid experiments.

\begin{claim}
\label{claim:hyb1-hyb2}
Suppose that the underlying $\AoK$ satisfies 
knowledge soundness, 
$\NIZK$ satisfies simulation sound extractability, 
and $\mcal{C}$ is probablistic polynomial-time, 
then $\mcal{C}$'s utility in $\Hyb_2$ has negligible statistical
distance from its utility in $\Hyb_1$.  
\end{claim}
\begin{proof}
The only difference between $\Hyb_2$ and $\Hyb_1$ is that $\Hyb_2$ 
runs an extractor alongside the main protocol, and it may abort
on some execution traces 
forcing the coalition $\mcal{C}$'s utility to be $0$.  
It is easy to see that 
if the $\AoK$ satisfies knowledge soundness
and 
$\NIZK$ 
satisfies simulation sound extractability, then the probability
of aborting is negligibly small.  
\end{proof}

%\elaine{TODO: insert a hybrid to show that the extracted
%vector consists of all honest commitments.}

\paragraph{Experiment $\Hyb_3$.}
$\Hyb_3$ is almost identical as $\Hyb_2$, except
that 
%if $i^*$ accepts the proof in the $\AoK_1$ of $\AoK_2$ instance, 
if all honest players accept the execution at the end, 
but 
the ${\bf c} := \{i, c_i, \pi_i\}_{i \in \mcal{I}}$
we have extracted 
from the $\AoK_1$ or $\AoK_2$ instance 
does not satisfy the following condition, 
\begin{itemize}
\item[]
every the honest buyer $j$'s tuple
$(j, c_j, \pi_j)$
is indeed contained in the extracted list ${\bf c}$,  
\end{itemize}
we abort and treat $\mcal{C}$'s utility as $0$. 

\begin{claim}
\label{claim:hyb2-hyb3}
Suppose that $\AoK$ satisfies knowledge soundness
and the hash family is collision resistant, 
\elaine{TO FIX: quasipoly}
then 
for a \ppt coalition $\mcal{C}$, its utility 
in $\Hyb_3$ has negligible statistical distance
from its utility in $\Hyb_2$. 
\end{claim}
\begin{proof}
It suffices to prove that 
in $\Hyb_2$, 
except with negligible probability, if all honest players accept the execution at the end, 
then every the honest buyer $j$'s tuple $(j, c_j, \pi_j)$
is indeed contained in the extracted list ${\bf c}$. 
Suppose this is not true. 
This means that there exists some honest $j \neq i^*$, 
such that on a non-negligible fraction of the execution traces, 
$i^*$ accepts the proof, but 
the tuple $(j, c_j, \pi_j)$ contributed by $j$ 
is not contained in the extracted list. 
We can then construct 
an efficient adversary  $\mcal{R}$ that produces a hash collision with non-negligible
probability assuming that the $\AoK$ scheme satisfies knowledge soundness. 
Essentially, $\mcal{R}$ runs the experiment $\Hyb_2$, but on the  side, it additionally
runs the extractor for the $\AoK_1$ or $\AoK_2$ instance   
where $j$ is the verifier, and let 
${\bf c}' || r'_{\mcal{P}}$ denote the extracted values. 
Due to the knowledge soundness of $\AoK$, 
except with negligible probability, if all honest players accept the execution at the end, 
it must be that 
${\bf c}' || r'_{\mcal{P}}$
is a valid witness to the corresponding NP statement, which implies
that 
$(j, c_j, \pi_j)$ must be contained in the extracted list ${\bf c}'$
and ${\sf digest} = h({\bf c}' || r'_{\mcal{P}})$. 
We also know that  
$(j, c_j, \pi_j)$ is not contained in ${\bf c}$
and ${\sf digest} = h({\bf c} || r_{\mcal{P}})$ --- note that if all honest players
accept at the end, it means that they must have received the same ${\sf digest}$ 
from the platform. 
This means that with non-negligible probability $\mcal{R}$ can output 
a hash collision 
${\bf c} || r_{\mcal{P}}$ 
and 
${\bf c}' || r'_{\mcal{P}}$. 
\end{proof}



\paragraph{Experiment $\Hyb_4$.}
$\Hyb_4$ is almost the same as $\Hyb_3$, 
except that when $\mcal{C}$ executes  
an instance of $\AoK_3$ (for buyers) or $\AoK_4$ (for sellers)
to prove 
that the auction's outcome 
is correctly computed w.r.t. the ${\sf digest}$, 
if all honest players accept the execution in the end, but there
exists some honest player 
(either a buyer or seller) such that the private outcome 
it receives is not the same as that computed
by running the honest rules $({\bf x},  {\bf p}, \mu_{\mcal{S}})$
over the following inputs and randomness: 
\hfill{($\heartsuit$)}
\begin{enumerate}[leftmargin=7mm,itemsep=1pt]
\item 
all honest buyers' true values 
$\{v_j\}_{j \in \mcal{H}}$; 
\item 
%the extracted values from the earlier $\AoK_1$ or $\AoK_2$ including  
the strategic buyer identities values 
$\{v_j\}_{j \in \mcal{I} \backslash \mcal{H}}$ 
extracted 
from the earlier $\AoK_1$ or $\AoK_2$ instance (where $i^*$ is the verifier); 
\item 
the random coin $r = 
\left(\displaystyle\mathop{\oplus}_{j \in \mcal{I}} r_j\right) \oplus r_\platform$
where 
the random coins 
$\{r_j\}_{j \in \mcal{I} \backslash \mcal{H}}$ 
and $r_\platform$ 
are extracted 
from the earlier $\AoK_1$ or $\AoK_2$ instance (where $i^*$ is the verifier),
and 
$\{r_j\}_{j \in \mcal{H}}$ 
denotes honest randomness that is sampled uniformly at random. 
\end{enumerate}
then abort and treat $\mcal{C}$'s utility as 0.  


\ignore{
to the first remaining honest player
denoted $j^*$ (which is either a buyer or seller), 
we additionally run the corresponding knowledge extractor
on the side to extract a witness 
$\left({\bf c}', {\bf r}_{\mcal{P}}', \mcal{I}, \{v'_j || j, 
{\sf coin}'_j\}_{j \in \mcal{I}}\right)$. 
Now, perform the following checks:  
\begin{itemize}[itemsep=1pt]
\item
If player $j^*$ accepts the proof but 
the witness is not valid, then abort and define $\mcal{C}$'s utility to be $0$.  
\item 
If $i^*$ 
accepted the proof in the $\AoK_1$ or $\AoK_2$ instance,
and $j^*$  
accepted the proof in the $\AoK_3$ or $\AoK_4$ instance,
but ${\bf c} \neq {\bf c}'$ or
${\bf r}_{\mcal{P}} \neq {\bf r}'_{\mcal{P}}$, then abort
and define $\mcal{C}$'s utility to be $0$.
\end{itemize}

Else, continue with the execution. 
}


\begin{claim}
\label{claim:hyb3-hyb4}
Suppose that the commitment scheme is perfectly binding, 
the $\AoK$  scheme satisfies 
knowledge soundness, 
the hash family is collision resistant, 
\elaine{TO FIX: quasipoly}
and $\mcal{C}$ is probablistic polynomial-time, 
then $\mcal{C}$'s utility in $\Hyb_4$ has negligible statistical
distance from its utility in $\Hyb_3$.  
\end{claim}
\begin{proof}
It suffices to show that except with negligible probability in $\Hyb_3$, 
if all honest players accept the execution at the end, 
then it must be that for every honest player, it receives a private outcome 
that is the same as 
running the honest auction rules on the inputs specified above. 

Suppose that this is not true. 
This means that there exists some honest player 
denoted $j^*$ (either a buyer or seller), such that 
with non-negligible probability, it receives an outcome 
that is different from the one computed using the honest auction rules
over the aforementioned inputs and randomness. 
We can construct the following  
efficient adversary $\mcal{R}$ that 
breaks the collision resistance of the hash function with non-negligible
probability, assuming that the $\AoK$ satisfies knowledge soundness and that
the commitment scheme is perfectly binding.
$\mcal{R}$ will run $\Hyb_3$, and alongside it will
invoke the extractor for the $\AoK_3$ or $\AoK_4$ instance
where $j^*$ is the verifier. 
Recall that $\AoK$ satisfies knowledge 
soundness. This means that except with negligible probability,
if all honest players accept the execution at the end, 
$\mcal{R}$ must extract a valid witness 
$(\mcal{I}', (j, c'_j, \pi'_j)_{j \in \mcal{I}'}, 
\{v'_j, r'_j, {\sf coin}'_j\}_{j \in \mcal{I}'}, r'_\platform)$
where 
every $(j \|v'_j \| r'_j, {\sf coin}'_j)$  is a valid opening
of the commitment $c'_j$, the outcome $j^*$
receives is 
computed from 
$\{v'_j\}_{j \in \mcal{I}'}$, 
and moreover, 
$h((j, c'_j, \pi'_j)_{j \in \mcal{I}'} || r'_{\mcal{P}}) = {\sf digest}$
where ${\sf digest}$ is the final digest posted to the blockchain. 
Because the commitment is perfectly binding, if 
$\{v'_j, r'_j\}_{j \in \mcal{I}'}$ is not the same
as the honest inputs $\{v_j\}_{j \in \mcal{H}}$
and the values $\{v_j, r_j\}_{j \in \mcal{I} \backslash \mcal{H}}$
extracted from $\AoK_1$ or $\AoK_2$, or if $\mcal{I} \neq \mcal{I}'$, 
it must be that 
$\{(j, c_j, \pi_j)\}_{j \in \mcal{I}} \neq 
\{(j, c'_j, \pi'_j)\}_{j \in \mcal{I}'}$. 
In this case $\mcal{R}$ can output a hash collision
$\{(j, c_j, \pi_j)\}_{j \in \mcal{I}} || r_{\mcal{P}}$
and 
$\{(j, c'_j, \pi'_j)\}_{j \in \mcal{I}'} || r'_{\mcal{P}}$. 
%\elaine{TODO: continue}
\end{proof}




\paragraph{Experiment $\Hyb_5$.}
$\Hyb_5$ is the same as $\Hyb_4$, except that if the experiment
does not abort, we now compute 
the coalition $\mcal{C}$'s utility as follows. 
Let $r_{\mcal{P}}$ and $\{j \|v_j\|r_j, {\sf coin}_j\}_{j \in \mcal{I}}$
be the extracted values from 
the extractor of either the $\AoK_1$ or $\AoK_2$ 
instance where $i^*$ is the verifier.
We will compute $\mcal{C}$'s utility by running 
the auction's rules $({\bf x}, {\bf p}, \mu_{\mcal{S}})$
over the inputs 
and randomness marked ($\heartsuit$) earlier. 
\ignore{
on 
the honest buyers' true values 
$\{v_j\}_{j \in \mcal{H}}$, 
honest randomness $\{r_j\}_{j \in \mcal{H}}$ that is sampled
uniformly at random, 
as well as 
the extracted values from $\AoK_1$ or $\AoK_2$ including  $\{v_j\}_{j \in \mcal{I} \backslash \mcal{H}}$ 
and ${\bf r}_{\mcal{P}}$, to compute the outcomes of all honest players.  
}
Given the honest players' outcomes
%the coalition $\mcal{C}$'s outcome
%(including the outcome of the platform, of all buyer identities
%in $\mcal{I} \backslash \mcal{H}$, 
%and possibly of the seller if the seller is part of the coalition)
%is also uniquely determined.  
and the true values of the buyers in $\mcal{C}$ (which may not
be equal to $\{v_j\}_{j \in \mcal{I} \backslash \mcal{H}}$), we can compute
$\mcal{C}$'s utility. 
If $\mcal{C}$'s utility computed in this way is less than $0$, we simply
set it to $0$.  


\begin{claim}
\label{claim:hyb4-hyb5}
$\mcal{C}$'s utility in $\Hyb_5$ 
stochastically dominates $\Hyb_4$.
\end{claim}
\begin{proof}
On traces where $i^*$  does not accept the $\AoK_1$ or $\AoK_2$ proof,
both experiments result in 0 utility for $\mcal{C}$.
On traces where $i^*$  accepts the $\AoK_1$ or $\AoK_2$ proof,
\begin{itemize}[itemsep=1pt]
\item 
if all honest players accept the execution in the end, %in $\Hyb_4$, 
then $\mcal{C}$'s utility in $\Hyb_5$ is greater than or equal
to its utility in $\Hyb_4$. The strictly greater case happens
when its utility in $\Hyb_4$ is negative and in $\Hyb_5$, it would be rounded up to $0$. 
%it is $\mcal{C}$'s utility in $\Hyb_4$ rounded up to 0;
\item 
if not all honest players accept the execution in the end in $\Hyb_4$,
then $\mcal{C}$'s utility in $\Hyb_5$ is at least 0 but  
$\mcal{C}$'s utility in $\Hyb_4$ 
is 0.
\end{itemize}
Therefore, the claim follows by the definition of stochastic dominance. 
\end{proof}

\paragraph{Experiment $\Hyb_6$.}
$\Hyb_6$ is the same as $\Hyb_5$, except with the following modifications.  
At  the beginning of the protocol, instead of having
honest buyers honestly committing to their true values, 
we instead commit to $0$.  
Note that at this point, the NIZK proofs  
are being simulated so we can still compute 
simulated NIZK proofs on behalf of
the honest buyers.
Note also that $\mcal{C}$'s utility is still computed using $(\heartsuit)$, 
%the honest buyers' true values 
%$\{v_j\}_{j \in \mcal{H}}$, as well as 
%the extracted values 
%$\{v_j\}_{j \in \mcal{I} \backslash \mcal{H}}$ 
%and ${\bf r}_{\mcal{P}}$, 
and its utility is lower bounded at $0$. 



\elaine{TO FIX: requires commitment to be secure against expected poly adv}
\elaine{TO FIX: change to quasi poly}
\begin{claim}
Suppose that commitment scheme is computationally hiding
for expected polynomial-time adversaries. Then, 
as long as $\mcal{C}$ is \ppt, its  
utility in $\Hyb_6$ is computationally indistinguishable from  
$\Hyb_5$.
\end{claim}
\begin{proof}
%\elaine{FILL}
Follows by a straightforward reduction to the computational hiding property of the commitment.  
\end{proof}

%\elaine{Finally, describe how hyb5 can be viewed as an ideal adv} 



\paragraph{Ideal auction and strategy.}
As long as there is at least one honest buyer or if the ideal auction's rules
are deterministic, 
then $\Hyb_6$ can equivalently be viewed as running ideal auction    
where the coalition $\mcal{C}$ that involves the platform
executes the following strategy:
\begin{enumerate}[leftmargin=8mm]
\item 
Honest buyers submit their true values to $\Fauction$ as bids, and strategic
buyers in the coalition do not send any bids. 
\item 
The strategic platform receives 
the number $n_H$ of honest bids from $\Fauction$. 
\item 
Invoke the real-world coalition's algorithm henceforth denoted $\mcal{C}$, 
and send to $\mcal{C}$ commitments of $0$,   
the honest identities, along with simulated proofs on behalf of 
$n_H$ honest buyers. 
Run the extractor to extract 
$\{v_j \| r_j \}_{j \in \mcal{I} \backslash \mcal{H}}$
and $r_{\mcal{P}}$
from $\AoK_1$ or $\AoK_2$. The strategic platform sends the extracted bids
$\{v_j\}_{j \in \mcal{I} \backslash \mcal{H}}$
to $\Fauction$. 
%\item 
%The strategic platform sends 
%the extracted ${\bf r}_{\mcal{P}}$
%to $\Fauction$. 
\item 
$\Fauction$ 
samples $r$ at random, and 
computes the auction's outcomes based on the rules $({\bf x}, {\bf p}, \mu_{\mcal{S}})$,
using all bids it has received and %the random coins ${\bf r}_\mcal{P}$. 
the randomness $r$.
$\Fauction$  now informs the strategic players their outcomes 
(including the outcomes of every buyer identity they submitted).
\item 
$\mcal{C}$ computes 
the utility of the coalition using the true values
of the buyers in the coalition. 
If this utility is less than $0$, $\mcal{C}$ instructs
$\Fauction$ to abort, 
otherwise it instructs $\Fauction$ to proceed. 
\end{enumerate}

\elaine{why do we need the platform to know everyone's outcomes in the ideal func?}
\elaine{TODO: fix ideal func, ideal func not correct}


\ignore{
\begin{claim}%[Utility dominance for strategic players]
For any \ppt coalition $\mcal{C}$ containing the platform,
its utility in the real-world execution 
is $(1-\negl(\lambda))$-almost-perfectly dominated
% computationally dominated
by its utility in expectation in the ideal world.  
\end{claim}
\begin{proof}
Due to the hybrid sequence above, 
we can see that 
the coalition's utility in the real execution and $\Hyb_4$ are computationally
indistinguishable. 
Its utility 
in $\Hyb_5$ 
stochastically dominates
its utility in 
$\Hyb_4$. 
Finally, its utilities in $\Hyb_5$ 
and in $\Hyb_6$ (same as the ideal world)
are computationally indistinguishable. 
The claim now follows from \Cref{lem:dominance-technical}. 
% the definition of computatinal dominance.
\end{proof}
}

Summarizing the above, $\mcal{C}$'s utility in the ideal world
computationally dominates its utility in the real world, 
as long as there is at least one honest buyer, or if the ideal auction's rules
are deterministic.


\subsubsection{Case 2: Platform is Honest}
\label{sec:proof-honest-platform}


\elaine{TO FIX: the experiment doesn't need to send 
hash to the adv before adv sends commitments}
%\elaine{TODO: continue editing here}

This is the easier case. 
The coalition 
$\mcal{C}$ 
consists either of one or more buyers, or just the seller.
Consider the following sequence of hybrid experiments. 

\paragraph{Experiment $\Hyb_1$.}
Replace the $\NIZK$'s setup with a simulated setup
which not only generates a simulated $\crs$ but also 
a trapdoor $\tau$ and 
an extraction key $\ek$.
When the honest platform 
needs to compute $\digest$, it needs to compute 
NIZK proofs on behalf of honest buyers.  
Instead of computing NIZK proofs honestly, we 
now use 
the trapdoor $\tau$ to compute simulated proofs without using the witness. 


\begin{claim}
Suppose that $\NIZK$ satisfies computational zero-knowledge
and the coalition $\mcal{C}$ is \ppt. 
The $\mcal{C}$'s utility in 
$\Hyb_1$ is computationally indistinguishable from 
its utility in 
the real execution.
\end{claim}
\begin{proof}
Follows from a straightforward reduction due to  
the computational zero-knowledge property of $\NIZK$.
\end{proof}

\paragraph{Experiment $\Hyb_2$.}
$\Hyb_2$ is almost the same as $\Hyb_1$, except
that the following modification.  
Suppose that the coalition 
sends 
the bid tuples $\{(j, c_j, \pi_j)\}_{j \in \mcal{B}^*}$
on behalf of the buyer-identities $\mcal{B}^*$.
Henceforth, we may assume that all the proofs $\{\pi_j\}_{j \in \mcal{B}^*}$ 
verify since
we simply discard the ones that do not verify.  
Let $\mcal{H}$ denote the honest buyers' identities.
If not all identities in $\mcal{B}^* \cup \mcal{H}$
are distinct, then perform random 
duplicate suppression. If 
an honest buyer's identity has been suppressed,
the experiment  
aborts and the coalition's utility is treated as $0$. 
Let $\mcal{B}$ be the set of 
non-honest identities after the duplicate suppression. 
At this moment, call the $\NIZK$'s extractor algorithm
using the extraction key $\ek$, and for each $j \in \mcal{B}$,
extract 
the opening $(j \| v_j \| r_j, \coin_j)$ to the commitment $c_j$. 
If the extracted value is not a valid opening, 
abort and let the coalition's utility be $0$. 
Otherwise, continue to execute the 
auction to the end. 
%Otherwise, run the honest auction rules
%$({\bf x}, {\bf p}, \mu_{\mcal{S}})$
%on the honest buyers' true values, 
%and the strategic bids $\{v_j\}_{j \in \mcal{B}}$, 
%using freshly sampled randomness. 

\begin{claim}
Suppose that the $\NIZK$ 
scheme
satisfies simulation sound extractability, and $\mcal{C}$ is \ppt. 
Then, $\mcal{C}$'s utility in $\Hyb_2$  
has negligible statistical distance from its utility 
in $\Hyb_1$.
\end{claim}
\begin{proof}
The only difference between $\Hyb_1$ and $\Hyb_2$ is that 
$\Hyb_2$ may abort 
if the extraction 
does not result in a valid witness for some $j \in \mcal{B}$
but the corresponding proof verifies. By the simulation
sound extractability of the $\NIZK$, this happens with negligible probability.
\end{proof}

\paragraph{Experiment $\Hyb_3$.}
$\Hyb_3$ is almost the same as $\Hyb_2$, except
that after the  
experiment sends the coalition $\mcal{C}$ the 
${\sf digest}$
of all committed bids 
on behalf of the honest platform, 
%after they perform   the ${\sf AoK}_1$ or ${\sf AoK}_2$ proofs, 
if some buyer identity $i^* \in \mcal{B}$ supplied by $\mcal{C}$ 
does not provide a valid opening to its previous commitment, 
abort and treat everyone's utility as $0$.
%we mark $i^*$ as aborted.
%We do not need to 
%continue the execution beyond 
%this point, and we simply determine the auction's outcome as follows. 
Otherwise, determine the auction's outcome as follows:
run the honest auction rules
$({\bf x}, {\bf p}, \mu_{\mcal{S}})$
on the honest buyers' true values, 
and the extracted strategic bids $\{v_j\}_{j \in \mcal{B}}$, 
using freshly sampled randomness. 

\begin{claim}
Suppose that the commitment scheme is perfectly binding, then  
the coalition's utility in $\Hyb_2$ 
is identically distributed from $\Hyb_3$. 
\end{claim}
\begin{proof}
The claim follows in a straightforward manner by observing the following:  
the only difference between $\Hyb_2$ and $\Hyb_3$ is that
in $\Hyb_2$, the coalition's utility is computed
using the the actual opened values from $\mcal{B}$, 
but in $\Hyb_3$, the coalition's utility is computed
using the extracted values.  
\end{proof}


\ignore{\paragraph{Experiment $\Hyb_3$.}
$\Hyb_3$ is almost the same as $\Hyb_2$, except
after extracting 
the openings for every $j \in \mcal{B}$, we do not continue with the auction,
we simply 
determine the outcome by 
running the honest auction rules
$({\bf x}, {\bf p}, \mu_{\mcal{S}})$
on the honest buyers' true values, 
and the strategic bids $\{v_j\}_{j \in \mcal{B}}$, 
using freshly sampled randomness. 



\begin{claim}
Suppose that the commitment scheme is perfectly binding, 
then the coalition's utility in $\Hyb_3$ stochastically
dominates its utility in $\Hyb_2$. 
\end{claim}
\begin{proof}
In $\Hyb_2$, the coalition may abort 
without opening their commitments which will cause
the auction to fail. 
However, in $\Hyb_3$, this will not happen.
The claim follows by the definition of stochastic dominance. 
\end{proof}
}


\paragraph{Experiment $\Hyb_4$.}
$\Hyb_4$ is almost the same as $\Hyb_3$ except
that when the platform needs
to compute $\digest$, %and perform an AoK proof
%with the coalition's identities $\mcal{B}$, 
we replace the honest buyers' commitments
with commitments of $0$.  
Recall that the honest buyers' NIZK
proofs have already been replaced
with simulated proofs, so we can still generate
these simulated proofs even if we are committing to $0$.  

\begin{claim}
Suppose that the commitment scheme is computationally hiding. 
Then,  the coalition's utility in $\Hyb_4$ 
is computationally indistinguishable from its utility in $\Hyb_3$.
\end{claim}
\begin{proof}
Follows from a straightforward reduction to the computational hiding property
of the commitment scheme. 
\end{proof}


\paragraph{Ideal auction and strategy.}
$\Hyb_4$ can be equivalently 
as running an ideal auction with the following strategy. 
%viewed as running the following strategy in the ideal auction. 
\begin{enumerate}[leftmargin=8mm]
\item 
Honest buyers submit their true values to $\Fauction$ as bids, and strategic
buyers in the coalition do not send any bids. 
\item 
$\Fauction$ sends the number %$n_H$ 
of honest bids to the platform, the coalition does not
receive anything. 
\item 
The ideal-world 
coalition's strategy is as follows. 
Interact 
with the real-world coalition's algorithm like in $\Hyb_4$.  
\ignore{
Wait for the real-world coalition's algorithm to submit  
the bid tuples $\{(c_j, j, \pi_j)\}_{j \in \mcal{B}^*}$, 
and then discard the tuples where the proofs do not verify and 
perform duplicate suppression. Let $\mcal{B}$ be the remaining non-honest
identities. 
Now, run the $\NIZK$ extractor to extract 
$\{v_j\}_{j \in \mcal{B}}$. 
}
%(after discarding duplicate identities and tuples where the proofs
%do not verify). 
%For identities in $\mcal{B}$ that are not marked as aborted,
%\elaine{platform needs to send digest and proof}
For the buyer identities $\mcal{B}$ belonging to the coalition, 
if they all provided a valid opening, 
then ideal-world coalition sends 
the extracted values $\{v_j\}_{j \in \mcal{B}}$ to $\Fauction$. 
Otherwise, send $0$ bids on behalf of $\mcal{B}$ to $\Fauction$
which implies that the coalition's utility is $0$. 
%Otherwise, send %arbitrary bids to $\Fauction$. 
%$\bot$ to $\Fauction$ causing the auction to abort. 
\item 
$\Fauction$ 
samples fresh randomness $r$ and 
computes the auction's outcomes 
based on the rules $({\bf x}, {\bf p}, \mu_{\mcal{S}})$,
using all bids it has received and the random coins $r$. 
$\Fauction$  now informs the strategic players their outcomes 
(including the outcomes of every buyer identity they submitted).
\item 
Platform sends ${\sf ok}$ and the auction is successful. 
\end{enumerate}

\begin{claim}
The coalition's utility is identically distributed
in $\Hyb_4$ and 
the ideal experiment. 
\end{claim}
\begin{proof}
Follows directly since the ideal experiment
is an equivalent rewrite of the 
$\Hyb_4$.
\end{proof}

%\paragraph{Experiment ${\sf Ideal}$.}

Summarizing the above, the coalition's utility in the real world
is computationally indistinguishable from its utility in the ideal
world.  
By \Cref{fct:indimpliesdom}, the coalition's utility in the real world 
is computationally dominated by its utility in the ideal world.
%\elaine{add fact to prelim, ind implies dom}

\ignore{
\begin{claim}%[Utility dominance for strategic players]
The \ppt coalition $\mcal{C}$'s utility 
in the real-world execution 
is $(1-\negl(\lambda))$-almost-perfectly dominated
% is computationally dominated 
by its utility in expectation in the ideal world.  
\elaine{TODO: fix, the defn also needs to be fixed.}
\end{claim}
\begin{proof}
The real-world utility is computationally 
indistinguishable from the utility in $\Hyb_2$. 
The utility in $\Hyb_3$ stochastically dominates $\Hyb_2$, 
and is identically distributed as the ideal world.
The claim now follows from 
\Cref{lem:dominance-technical}.
% the definition of computatioanl dominance.
\end{proof}
}


==> psIC-multiround-hao.tex <==
\subsection{bIC + psIC $\Longrightarrow$ Small Revenue (Information-Theoretic)}

In this section,
we consider the case where the players are computationally unbounded.
We assume that the auction must terminate at most in $t$ rounds, 
where $t$ is a pre-determined parameter independent of buyers' values.
We also assume each player has access to its random tape,
which is uniformly sampled from $\{0,1\}^{t\cdot \ell}$,
where $\ell$ is the number of random bits used for each round.
% We also assume the players' protocol messages can be represented by $\ell$-bit strings,
% regardless of private or public communication.
% These assumptions imply the auction is a \emph{finite} game among the platform,
% the seller, and all buyers.

% Consider any auction $\Pi_\lambda$ parametrized by the security parameter $\lambda$.
% We assume the number of rounds of interaction (including private and public communication) 
% between the platform and any buyer is bounded by a polynomial $t(\lambda)$.
% When the auction is randomized, 
% we assume all players have access to a $\ell(\lambda)$-bit random tape at each round, 
% where $\ell(\lambda)$ is a polynomial in $\lambda$.

\begin{definition}[Revenue dominated by posted price]
%\elaine{TODO: parametrize by lambda}
Let $\Pi_\lambda$ be an auction parametrized by $\lambda$ 
over the value domain $\inDomSecu$. 
We say that $\Pi_\lambda$ 
is $\delta(\cdot)$-revenue dominated by posted
price %w.r.t. to the value distribution $\mcal{D}$, 
iff 
	every $\lambda$, 
there exist some $r_\lambda$ such that 
for any bid vector ${\bf b} \in \inDomSecu^*$, %of polynomial length,
$\Pi_\lambda$'s 
expected total payment under ${\bf b}$ 
is at most $\delta(\lambda)$ more than 
``the posted price auction
with reserve $r_\lambda$'' under ${\bf b}$. 
For the special case where $\delta(\lambda) = 0$ for all $\lambda$,
	we also simply say
that the 
auction is (strictly) revenue dominated by posted price. 
\end{definition}

	
	
\begin{theorem}[bIC + psIC $\Longrightarrow$ small revenue]
Consider any auction $\Pi_\lambda$ where buyers' values are in a finite value domain $\inDom \subset [0, 1]$. 
Suppose $\Pi_\lambda$ satisfies information theoretic bIC and psIC simultaneously.
Then, the auction  
must be strictly revenue dominated by posted price. 
% \elaine{fix this after fixing the IT defn}
\label{thm:psic-multiround-imp}
\end{theorem}

\paragraph{Proof of \cref{thm:psic-multiround-imp}.}
\hao{Need to show the outcome can be uniquely determined by the protocol messages, i.e.~the transcript.}

\hao{
Proof sketch:
We say a message is \emph{decisive} if the outcome is fixed after this message.
In more detail, no matter which protocol messages are sent after the decisive message,
the outcomes do not change.
There are three possibilities:
1) the first message (true value $v$) is decisive;
2) some platform's message (randomness) is decisive;
3) some buyer's message (other than the first true value) (randomness) is decisive.

The second case implies the payment is always zero.
The third case implies the payment is always the same as the true value.

The third case can be further divided into two subcases:
3-1) the allocation probability is zero.
3-2) the allocation probability is 1, but the payment is the same as the true value.

It is impossible two have $b, b' >$ such that $b' > b$, and both $b,b'$ lead to 3-2.
Otherwise, the buyer with value $b'$ can underbid $b$.
}


Consider a scenario where there is only one buyer with true value $v$.
Without loss of generality, we may assume the auction $\Pi_\lambda$ is executed as follows:
1) the auction always proceeds in $t$ rounds;
2) in each round $i$, the buyer sends a message $m_i$ to the platform, 
where $m_i$ may depend on its true value $v$, the buyer's randomness $r_i \in \{0,1\}^\ell$, and all previous messages;
and 3) in each round $i$,
after receiving $m_i$ from the buyer, the platform sends a message $m'_i$ to the buyer,
where $m'_i$ may depend on the platform's randomness $r'_i \in \{0,1\}^\ell$, and the transcript of the previous rounds.
\hao{How to integrate public communication cleanly in the assumption?}
% and 3) in each round $i$, the buyer's message may depend on its true value $v$, its randomness $r_i \in \{0,1\}^{\ell}$ for round $i$, 
% and the transcript of all previous rounds;
% similarly, the platform's message may depend on its randomness $r'_i \in \{0,1\}^{\ell}$, and the transcript of the previous rounds.
This assumption is without loss of generality because we can always pad dummy messages 
if the actual auction ends before $t$ rounds.

Next, given $\Pi_\lambda$, we construct the \emph{canonical auction} of $\Pi_\lambda$ as follows.
\begin{itemize}
\item 
At round $0$, the buyer sends its true value $v$ to the platform.
\item 
At round $i = 1,\cdots,t$,
the buyer sends its randomness $r_i$ to the platform,
and the platform sends its randomness $r'_i$ to the buyer.
\item 
The outcome is computed as if the buyer and the platform
follow the protocol of $\Pi_\lambda$ using the value $v$ and the randomness $(r_1,\cdots,r_t,r'_1,\cdots,r'_t)$.
\end{itemize}

It is easy to see that for any buyer's true value $v$,
the expected outcome of $\Pi_\lambda$ is identically distributed as the canonical auction,
where the randomness is taken over the choices of $(r_1,\cdots,r_t,r'_1,\cdots,r'_t)$.

\begin{claim}
If $\Pi_\lambda$ satisfies information theoretic bIC and psIC,
then the canonical auction must also satisfy information theoretic bIC and psIC.
\end{claim}
\begin{proof}
% For the sake of contradiction,
% suppose $\Pi'_\lambda$ does not satisfy information theoretic bIC.
% That is, there exist a value $v$, random tape $\bfr = (r_1,\cdots,r_t)$ 
% and a strategy $S'$ such that 
% the buyer can profit by deviating from $\Pi'_\lambda$ when it starts with $v$ and $\bfr$.
% Then, imagine the case where the buyer starts with $v$ and $\bfr$ in $\Pi_\lambda$.
Given any strategy $S'$ for the buyer in the canonical auction,
we can construct a strategy $S$ for the buyer in $\Pi_\lambda$ as follows:
\begin{itemize}
\item 
At round $0$, the buyer sends $v'$ to the platform,
where $v'$ is the value that $S'$ sends in the canonical auction.
\item 
At round $i = 1,\cdots,t$,
$S'$ outputs a strategically chosen randomness $r_i$.
$S$ sends $m_i$ to the platform, where $m_i$ depends on $v'$, the strategic randomness $r_i$, 
and all previous messages.
Then, on receiving $m'_i$ from the platform,
$S$ computes the set $\mcal{R}'_i$ of all possible randomness that can lead to $m'_i$
assuming the platform is honest.
$S$ randomly chooses $r'_i$ from $\mcal{R}'_i$, and sends $r'_i$ to $S'$.
\end{itemize}
The expected utility of the buyer in $\Pi_\lambda$ when adopting $S$ 
is identically distributed as the expected utility in the canonical auction when adopting $S'$.
Thus, if $\Pi_\lambda$ satisfies information theoretic bIC,
then the canonical auction must also satisfy information theoretic bIC.
The proof for psIC is similar.
\end{proof}

Now, consider the transcript $\trans = (v,r_1,r'_1,\cdots,r_t,r'_t)$ of any canonical auction.
We say a protocol message $m \in \trans$ is \emph{decisive} if 
$m$ is the earliest message such that the outcome is fixed after $m$;
in other words, given the protocol execution up to $m$,
the outcome does not change no matter what messages are sent after $m$,
while the outcome may change if we replace $m$ with a different protocol message $m'$.

For any auction that satisfies information theoretic bIC,
at any round $i = 1,\cdots,t$,
conditioned on the protocol messages up to round $i-1$,
the buyer's expected utility should be the same for any protocol message $r_i \in \{0,1\}^\ell$,
where the expectation is taken over the randomness $(r_{i+1}, \dots, r_t, r'_i, \dots, r'_t)$.
Otherwise, the buyer is incentivized to strategically choose $r_i$ to profit.
The same argument applies to the platform according to psIC.

Consider any transcript $\trans = (v,r_1,r'_1,\cdots,r_t,r'_t)$ of any canonical auction. 
There are three possibilities.
\begin{itemize}
\item 
{\bf Case 1:}
The buyer's value $v$ at round $0$ is decisive.
\item 
{\bf Case 2:}
The buyer's randomness $r_i$ at round $i$ is decisive.
\item 
{\bf Case 3:}
The platform's randomness $r'_i$ at round $i$ is decisive.
\end{itemize}
If it is Case 2,
then the buyer's utility at round $i$ must be zero regardless of the messages $r_i$ the buyer sends.


% Next, let $\Pi'_\lambda$ be the auction which is the same as $\Pi_\lambda$ except that 
% the buyer directly sends its true value $v$ to the platform at the beginning of the auction.
% If $\Pi_\lambda$ satisfies bIC and psIC,
% then $\Pi'_\lambda$ must also satisfy bIC and psIC.
% Otherwise, if $\Pi'_\lambda$ does not satisfy psIC,
% there exists a strategy $S$ such that the platform-seller coalition is incentivized 
% to deviate from the auction
% after observing the buyer's true value $v$,
% while psIC requires the platform-seller coalition cannot profit by deviation
% for any buyer's true value $v \in \inDom$.
% % the platform-seller coalition must be able to profit on receiving the first message $b$ for the buyer.
% % Consequently, the platform-seller coalition can also profit in $\Pi_\lambda$ when the buyer's true value is $v$.
% On the other hand, $\Pi'_\lambda$ satisfies bIC
% because the honest platform does not use the first message in $\Pi'_\lambda$.
% % if $\Pi'_\lambda$ does not satisfy bIC,
% % the buyer can adopt the same strategy in $\Pi_\lambda$ to profit
% % because the honest platform does not use the first message in $\Pi'_\lambda$.
% Because this first message is not used in $\Pi'_\lambda$,
% the expected payment in $\Pi'_\lambda$ is the same as in $\Pi_\lambda$
% when both the buyer and the platform follow the auction honestly.

\iffalse
Next, given any auction $\Pi_\lambda$ where the only buyer always 
sends its true value $v$ to the platform at the beginning of the auction.
We construct another auction $\Pi'_\lambda$ as follows.
At the beginning of the auction, the buyer sends its true value $v$ to the platform.
Then, at each round $i$, the buyer sends its randomness $r_i$ to the platform,
and the platform sends its randomness $r'_i$ to the buyer.
At the end, the outcome of $\Pi'_\lambda$ is computed according to the same rule as $\Pi_\lambda$ 
using the randomness $(r_1,\cdots,r_{t(\lambda)},r'_1,\cdots,r'_{t(\lambda)})$.

\begin{claim}
\label{claim:random-equivalence}
Suppose there is only one buyer in the auction.
If $\Pi_\lambda$ satisfies computational bIC and computational psIC,
then $\Pi'_\lambda$ must also satisfy computational bIC and computational psIC.
\end{claim}
\begin{proof}[Proof of \cref{claim:random-equivalence}]
We prove the case of computational bIC, since the case of computational psIC is similar.
Let $U_\lambda(v)$ be the expected utility of the buyer in $\Pi'_\lambda$ when its true value is $v$
in the honest execution.
For the sake of contradiction, suppose $\Pi'_\lambda$ does not satisfy computational bIC.
That is, for infinitely many $\lambda$'s, 
there is a value $v_\lambda \in \inDomSecu$
\end{proof}
\fi

In the rest of the proof, 
we focus on an auction where the honest buyer always sends its true value $v$ to the platform at the beginning of the auction.
% Additionally, we assume that the strategic buyer and the platform 
% only choose the randomness $\bfr, \bfr'$ strategically,
% while they follow the protocol honestly otherwise.

\begin{claim}
\label{claim:buyer-strategy}
Suppose the world has only one buyer with an arbitrary value $b \in \inDomSecu$. 
There exists a negligible function $\negl$ such that
except over negligible probability
over the choice of $\bfr \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
$|{\sf butil}(\bfr,b) - {\sf butil}(b)| \leq \negl(\lambda)$,
where ${\sf butil}(\bfr,b)$ denotes the buyer's expected utility conditioned on randomness $\bfr$ and the value $b$,
and ${\sf butil}(b)$ denotes the buyer's expected utility given value $b$,
assuming the platform follows the protocol honestly.
% \label{clm:psic-msg}
\end{claim}
\begin{proof}
For the same of contradiction, 
suppose for infinitely many $\lambda$'s, 
there is some $b_\lambda \in \inDomSecu$, such that 
with at least $1/\poly(\lambda)$ probability over
the choice of $\bfr$, we have
$|{\sf butil}(\bfr, b_\lambda) - {\sf butil}(b_\lambda)| \geq 1/\poly(\lambda)$. 
Below, we omit 
writing ``for infinitely many $\lambda$'s'' whenever the context is clear. 
By \Cref{fct:deviate}, 
it must be that with at least $1/\poly_1(\lambda)$ probability
over $\bfr$, 
${\sf butil}(\bfr,b_\lambda) - {\sf butil}(b_\lambda) \geq 1/\poly_1(\lambda)$.
Now a strategic buyer 
with value $b_\lambda$ can simply choose
a $\bfr$ 
such that ${\sf butil}(\bfr,b_\lambda) - {\sf butil}(b_\lambda) \geq 1/\poly_1(\lambda)$, 
and such a random tape $\bfr$ can be provided to the buyer as an advice string. \hao{Non-uniform advice!}
This strategy will let the buyer gain 
$1/\poly_1(\lambda)$ amount over the honest strategy,
which violates computational bIC. 
\end{proof}

\begin{claim}
\label{claim:platform-strategy}
Suppose the world has only one buyer with an arbitrary value $b \in \inDomSecu$. 
There exists a negligible function $\negl$ such that
except over negligible probability
over the choice of $\bfr' \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
$|\mu(\bfr',b) - \mu(b)| \leq \negl(\lambda)$,
where $\mu(\bfr',b)$ denotes the expected payment conditioned on $\bfr'$,
and $\mu(b)$ denotes the expected payment given value $b$,
assuming the buyer follows the protocol honestly.
% \label{clm:psic-msg}
\end{claim}
\begin{proof}
For the same of contradiction, 
suppose for infinitely many $\lambda$'s, 
there is some $b_\lambda \in \inDomSecu$, such that 
with at least $1/\poly(\lambda)$ probability over
the choice of $\bfr'$, we have
$|\mu(\bfr', b) - \mu(b_\lambda)| \geq 1/\poly(\lambda)$. 
Below, we omit 
writing ``for infinitely many $\lambda$'s'' whenever the context is clear. 
By \Cref{fct:deviate}, 
it must be that with at least $1/\poly_1(\lambda)$ probability
over $\bfr'$, 
$\mu(\bfr',b) - \mu(b_\lambda) \geq 1/\poly_1(\lambda)$.
Now the strategic platform can choose $\bfr'$ 
such that $\mu(\bfr',b) - \mu(b_\lambda) \geq 1/\poly_1(\lambda)$, 
and such a random tape $\bfr'$ can be provided to the buyer as an advice string. \hao{Non-uniform advice!}
This strategy will let the buyer gain 
$1/\poly_1(\lambda)$ amount over the honest strategy,
which violates computational psIC. 
\end{proof}


Fix some $\lambda$.
Let $\negl'(\cdot)$ be a negligible function whose value sufficiently large 
w.r.t.~the negligible functions in \Cref{clm:helperpsic}
for sufficiently large $\lambda$s. 
Then, for any $b_\lambda \in \inDomSecu$,
assuming the buyer honestly sends the true value $b_\lambda$ to the platform
at the beginning of the auction,
over the choice of $\bfr \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
and $\bfr' \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
it must fall into one of the following two cases:
\begin{itemize}[leftmargin=6mm,itemsep=1pt]
\item 
{\bf Case 1:} 
the buyer does not get an item with probability at least $\negl'(\lambda)$;
\item 
{\bf Case 2:} 
the buyer gets an item with probability at least $1-\negl'(\lambda)$.
\end{itemize}

For any $b_\lambda$ that falls into Case 1,
except with negligible fraction of the choice of $\bfr \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
the buyer's expected payment is at most $\negl(\lambda)$ by \cref{claim:buyer-strategy}.
For any $b_\lambda$ that falls into Case 2,
except with negligible fraction of the choice of $\bfr' \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
the buyer's expected payment is at most $\mu(b_\lambda) + \negl(\lambda)$ by \cref{claim:platform-strategy}.

Next, it must be that for any $b_\lambda, b'_\lambda$ that fall into Case 2,
it must be $|\mu(b_\lambda) - \mu(b'_\lambda)| \leq \negl(\lambda)$.
Otherwise, suppose $|\mu(b_\lambda) - \mu(b'_\lambda)| > \poly(\lambda)$.
If $\mu(b_\lambda) > \mu(b'_\lambda)$, then the buyer with value $b_\lambda$ can pretend to have value $b'_\lambda$.
Because the allocation probability can only reduce by at most $\negl'(\lambda)$,
its utility gain is $\poly(\lambda) - \negl'(\lambda)$, which violates computational bIC.
The case of $\mu(b_\lambda) < \mu(b'_\lambda)$ is similar.

% Finally, we can set $r_\lambda$ to be the reserve price that is the closest to $\mu(b_\lambda)$.
Finally, suppose that for infinitely many $\lambda$'s, 
there is bid vector ${\bf b} = (b_1, \ldots, b_n) \in \inDomSecu^n$ 
such that some buyer $i$'s expected payment is more than 
$\mu_\lambda + 1 /\poly(\lambda)$.
We have the following
scenario and strategy 
that violate computational psIC.
Suppose the world actually has only a single buyer 
with true value $b_i$.
The platform-seller  
pretends that the world is actually ${\bf b}$ where
the victim buyer is the $i$-th coordinate. 
In other words, the strategy will simulate
$n-1$ fake players with the true values $\bfb_{-i}$
and run the protocol with the single victim buyer. 
This strategy has expected gain at least $1/\poly(\lambda) - \negl(\lambda)$.
This violates 
computational psIC. 

For the information-theoretic case, we can force all the negligible functions
to be $0$. In this case, all the $1/\poly(\lambda)$ slacks would vanish to $0$, 
and the statement follows directly. 




\iffalse
\subsection{bIC + psIC $\Longrightarrow$ Small Revenue}

Consider any auction $\Pi_\lambda$ parametrized by the security parameter $\lambda$.
We assume the number of rounds of interaction (including private and public communication) 
between the platform and any buyer is bounded by a polynomial $t(\lambda)$.
When the auction is randomized, 
we assume all players have access to a $\ell(\lambda)$-bit random tape at each round, 
where $\ell(\lambda)$ is a polynomial in $\lambda$.

\begin{definition}[Revenue dominated by posted price]
%\elaine{TODO: parametrize by lambda}
Let $\Pi_\lambda$ be an auction parametrized by $\lambda$ 
over the value domain $\inDomSecu$. 
We say that $\Pi_\lambda$ 
is $\delta(\cdot)$-revenue dominated by posted
price %w.r.t. to the value distribution $\mcal{D}$, 
iff 
	every $\lambda$, 
there exist some $r_\lambda$ such that 
for any bid vector ${\bf b} \in \inDomSecu^*$, %of polynomial length,
$\Pi_\lambda$'s 
expected total payment under ${\bf b}$ 
is at most $\delta(\lambda)$ more than 
``the posted price auction
with reserve $r_\lambda$'' under ${\bf b}$. 
For the special case where $\delta(\lambda) = 0$ for all $\lambda$,
	we also simply say
that the 
auction is (strictly) revenue dominated by posted price. 
\end{definition}

	
	
\begin{theorem}[bIC + psIC $\Longrightarrow$ small revenue]
Consider any auction $\Pi_\lambda$ parametrized by $\lambda$,
where buyers' values are in the value domain $\inDomSecu \subset [0, 1]$. 
Suppose $\Pi_\lambda$ satisfies computational bIC and computational psIC
simultaneously.
Then, 
there exists a negligible function $\negl(\cdot)$, such that 
for every $\lambda$, 
$\Pi_\lambda$
is $\negl(\lambda)$-revenue dominated by posted price. 

Further, if ``computational'' is replaced with ``information theoretic'' above,
then the auction  
must be strictly revenue dominated by posted price. 
\elaine{fix this after fixing the IT defn}
\label{thm:psic-multiround-imp}
\end{theorem}

\paragraph{Proor of \cref{thm:psic-multiround-imp}.}

Consider a scenario where there is only one buyer with true value $v$.
Without loss of generality, we may assume the auction $\Pi_\lambda$ is executed as follows:
1) the auction always proceeds in $t(\lambda)$ rounds;
and 2) in each round, the buyer sends a message to the platform, and the platform replies a message to the buyer.
% and 3) in each round $i$, the buyer's message may depend on its true value $v$, its randomness $r_i \in \{0,1\}^{\ell(\lambda)}$ for round $i$, 
% and the transcript of all previous rounds;
% similarly, the platform's message may depend on its randomness $r'_i \in \{0,1\}^{\ell(\lambda)}$, and the transcript of the previous rounds.
This assumption is without loss of generality because we can always pad dummy messages 
if the actual auction ends before $t(\lambda)$ rounds.

Next, let $\Pi'_\lambda$ be the auction which is the same as $\Pi_\lambda$ except that 
the buyer directly sends its true value $v$ to the platform at the beginning of the auction.
If $\Pi_\lambda$ satisfies computational bIC and computational psIC,
then $\Pi'_\lambda$ must also satisfy computational bIC and computational psIC.
Otherwise, if $\Pi'_\lambda$ does not satisfy computational psIC,
there exists a strategy $S$ such that the platform-seller coalition can profit by $\poly(\lambda)$
after observing the buyer's true value $v$.
% the platform-seller coalition must be able to profit on receiving the first message $b$ for the buyer.
Consequently, the platform-seller coalition can also profit in $\Pi_\lambda$ when the buyer's true value is $v$.
On the other hand, $\Pi'_\lambda$ satisfies computational bIC
because the honest platform does not use the first message in $\Pi'_\lambda$.
% if $\Pi'_\lambda$ does not satisfy computational bIC,
% the buyer can adopt the same strategy in $\Pi_\lambda$ to profit
% because the honest platform does not use the first message in $\Pi'_\lambda$.
Because this first message is not used in $\Pi'_\lambda$,
the expected payment in $\Pi'_\lambda$ is the same as in $\Pi_\lambda$
when both the buyer and the platform follow the auction honestly.

\iffalse
Next, given any auction $\Pi_\lambda$ where the only buyer always 
sends its true value $v$ to the platform at the beginning of the auction.
We construct another auction $\Pi'_\lambda$ as follows.
At the beginning of the auction, the buyer sends its true value $v$ to the platform.
Then, at each round $i$, the buyer sends its randomness $r_i$ to the platform,
and the platform sends its randomness $r'_i$ to the buyer.
At the end, the outcome of $\Pi'_\lambda$ is computed according to the same rule as $\Pi_\lambda$ 
using the randomness $(r_1,\cdots,r_{t(\lambda)},r'_1,\cdots,r'_{t(\lambda)})$.

\begin{claim}
\label{claim:random-equivalence}
Suppose there is only one buyer in the auction.
If $\Pi_\lambda$ satisfies computational bIC and computational psIC,
then $\Pi'_\lambda$ must also satisfy computational bIC and computational psIC.
\end{claim}
\begin{proof}[Proof of \cref{claim:random-equivalence}]
We prove the case of computational bIC, since the case of computational psIC is similar.
Let $U_\lambda(v)$ be the expected utility of the buyer in $\Pi'_\lambda$ when its true value is $v$
in the honest execution.
For the sake of contradiction, suppose $\Pi'_\lambda$ does not satisfy computational bIC.
That is, for infinitely many $\lambda$'s, 
there is a value $v_\lambda \in \inDomSecu$
\end{proof}
\fi

In the rest of the proof, 
we focus on an auction where the honest buyer always sends its true value $v$ to the platform at the beginning of the auction.
% Additionally, we assume that the strategic buyer and the platform 
% only choose the randomness $\bfr, \bfr'$ strategically,
% while they follow the protocol honestly otherwise.

\begin{claim}
\label{claim:buyer-strategy}
Suppose the world has only one buyer with an arbitrary value $b \in \inDomSecu$. 
There exists a negligible function $\negl$ such that
except over negligible probability
over the choice of $\bfr \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
$|{\sf butil}(\bfr,b) - {\sf butil}(b)| \leq \negl(\lambda)$,
where ${\sf butil}(\bfr,b)$ denotes the buyer's expected utility conditioned on randomness $\bfr$ and the value $b$,
and ${\sf butil}(b)$ denotes the buyer's expected utility given value $b$,
assuming the platform follows the protocol honestly.
% \label{clm:psic-msg}
\end{claim}
\begin{proof}
For the same of contradiction, 
suppose for infinitely many $\lambda$'s, 
there is some $b_\lambda \in \inDomSecu$, such that 
with at least $1/\poly(\lambda)$ probability over
the choice of $\bfr$, we have
$|{\sf butil}(\bfr, b_\lambda) - {\sf butil}(b_\lambda)| \geq 1/\poly(\lambda)$. 
Below, we omit 
writing ``for infinitely many $\lambda$'s'' whenever the context is clear. 
By \Cref{fct:deviate}, 
it must be that with at least $1/\poly_1(\lambda)$ probability
over $\bfr$, 
${\sf butil}(\bfr,b_\lambda) - {\sf butil}(b_\lambda) \geq 1/\poly_1(\lambda)$.
Now a strategic buyer 
with value $b_\lambda$ can simply choose
a $\bfr$ 
such that ${\sf butil}(\bfr,b_\lambda) - {\sf butil}(b_\lambda) \geq 1/\poly_1(\lambda)$, 
and such a random tape $\bfr$ can be provided to the buyer as an advice string. \hao{Non-uniform advice!}
This strategy will let the buyer gain 
$1/\poly_1(\lambda)$ amount over the honest strategy,
which violates computational bIC. 
\end{proof}

\begin{claim}
\label{claim:platform-strategy}
Suppose the world has only one buyer with an arbitrary value $b \in \inDomSecu$. 
There exists a negligible function $\negl$ such that
except over negligible probability
over the choice of $\bfr' \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
$|\mu(\bfr',b) - \mu(b)| \leq \negl(\lambda)$,
where $\mu(\bfr',b)$ denotes the expected payment conditioned on $\bfr'$,
and $\mu(b)$ denotes the expected payment given value $b$,
assuming the buyer follows the protocol honestly.
% \label{clm:psic-msg}
\end{claim}
\begin{proof}
For the same of contradiction, 
suppose for infinitely many $\lambda$'s, 
there is some $b_\lambda \in \inDomSecu$, such that 
with at least $1/\poly(\lambda)$ probability over
the choice of $\bfr'$, we have
$|\mu(\bfr', b) - \mu(b_\lambda)| \geq 1/\poly(\lambda)$. 
Below, we omit 
writing ``for infinitely many $\lambda$'s'' whenever the context is clear. 
By \Cref{fct:deviate}, 
it must be that with at least $1/\poly_1(\lambda)$ probability
over $\bfr'$, 
$\mu(\bfr',b) - \mu(b_\lambda) \geq 1/\poly_1(\lambda)$.
Now the strategic platform can choose $\bfr'$ 
such that $\mu(\bfr',b) - \mu(b_\lambda) \geq 1/\poly_1(\lambda)$, 
and such a random tape $\bfr'$ can be provided to the buyer as an advice string. \hao{Non-uniform advice!}
This strategy will let the buyer gain 
$1/\poly_1(\lambda)$ amount over the honest strategy,
which violates computational psIC. 
\end{proof}


Fix some $\lambda$.
Let $\negl'(\cdot)$ be a negligible function whose value sufficiently large 
w.r.t.~the negligible functions in \Cref{clm:helperpsic}
for sufficiently large $\lambda$s. 
Then, for any $b_\lambda \in \inDomSecu$,
assuming the buyer honestly sends the true value $b_\lambda$ to the platform
at the beginning of the auction,
over the choice of $\bfr \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
and $\bfr' \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
it must fall into one of the following two cases:
\begin{itemize}[leftmargin=6mm,itemsep=1pt]
\item 
{\bf Case 1:} 
the buyer does not get an item with probability at least $\negl'(\lambda)$;
\item 
{\bf Case 2:} 
the buyer gets an item with probability at least $1-\negl'(\lambda)$.
\end{itemize}

For any $b_\lambda$ that falls into Case 1,
except with negligible fraction of the choice of $\bfr \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
the buyer's expected payment is at most $\negl(\lambda)$ by \cref{claim:buyer-strategy}.
For any $b_\lambda$ that falls into Case 2,
except with negligible fraction of the choice of $\bfr' \getr \{0,1\}^{r(\lambda) \cdot t(\lambda)}$,
the buyer's expected payment is at most $\mu(b_\lambda) + \negl(\lambda)$ by \cref{claim:platform-strategy}.

Next, it must be that for any $b_\lambda, b'_\lambda$ that fall into Case 2,
it must be $|\mu(b_\lambda) - \mu(b'_\lambda)| \leq \negl(\lambda)$.
Otherwise, suppose $|\mu(b_\lambda) - \mu(b'_\lambda)| > \poly(\lambda)$.
If $\mu(b_\lambda) > \mu(b'_\lambda)$, then the buyer with value $b_\lambda$ can pretend to have value $b'_\lambda$.
Because the allocation probability can only reduce by at most $\negl'(\lambda)$,
its utility gain is $\poly(\lambda) - \negl'(\lambda)$, which violates computational bIC.
The case of $\mu(b_\lambda) < \mu(b'_\lambda)$ is similar.

% Finally, we can set $r_\lambda$ to be the reserve price that is the closest to $\mu(b_\lambda)$.
Finally, suppose that for infinitely many $\lambda$'s, 
there is bid vector ${\bf b} = (b_1, \ldots, b_n) \in \inDomSecu^n$ 
such that some buyer $i$'s expected payment is more than 
$\mu_\lambda + 1 /\poly(\lambda)$.
We have the following
scenario and strategy 
that violate computational psIC.
Suppose the world actually has only a single buyer 
with true value $b_i$.
The platform-seller  
pretends that the world is actually ${\bf b}$ where
the victim buyer is the $i$-th coordinate. 
In other words, the strategy will simulate
$n-1$ fake players with the true values $\bfb_{-i}$
and run the protocol with the single victim buyer. 
This strategy has expected gain at least $1/\poly(\lambda) - \negl(\lambda)$.
This violates 
computational psIC. 

For the information-theoretic case, we can force all the negligible functions
to be $0$. In this case, all the $1/\poly(\lambda)$ slacks would vanish to $0$, 
and the statement follows directly. 
\fi
